Filtering DDoS Attacks from Unlabeled Network Traffic Data Using Online Deep Learning

DDoS attacks are simple, effective, and still pose a significant threat even after more than two decades. Given the recent success in machine learning, it is interesting to investigate how we can leverage deep learning to filter out application layer attack requests. There are challenges in adopting deep learning solutions due to the ever-changing profiles, the lack of labeled data, and constraints in the online setting. Offline unsupervised learning methods can sidestep these hurdles by learning an anomaly detector $N$ from the normal-day traffic ${\mathcal N}$. However, anomaly detection does not exploit information acquired during attacks, and their performance typically is not satisfactory. In this paper, we propose two frameworks that utilize both the historic ${\mathcal N}$ and the mixture ${\mathcal M}$ traffic obtained during attacks, consisting of unlabeled requests. We also introduce a machine learning optimization problem that aims to sift out the attacks using ${\mathcal N}$ and ${\mathcal M}$. First, our proposed approach, inspired by statistical methods, extends an unsupervised anomaly detector $N$ to solve the problem using estimated conditional probability distributions. We adopt transfer learning to apply $N$ on ${\mathcal N}$ and ${\mathcal M}$ separately and efficiently, combining the results to obtain an online learner. Second, we formulate a specific loss function more suited for deep learning and use iterative training to solve it in the online setting. On publicly available datasets, our online learners achieve a $99.3\%$ improvement on false-positive rates compared to the baseline detection methods. In the offline setting, our approaches are competitive with classifiers trained on labeled data.

==> section/old_sec1-intro.tex <==
%-------------------------------------------------------------------------------
\section{Introduction}
%-------------------------------------------------------------------------------
% ======== [1. Introduce the problem] ======== 
% [version 1]
% Distributed Denial-of-Service (DDoS) attacks are well established as a significant threat to the network security of our present-day Internet, denying legitimate users access to shared and essential resources alike. The earliest reported DDoS attack in 1999~\cite{criscuolo2000distributed} started a wave of denial-of-service attacks that are distributed in nature. One of the latest methods popular with malicious agents is to launch an attack by remotely controlling a network of well organized, and widely distributed Botnet devices.
% %~\afterpage{\footnote{Devices such as computers, smartphones, and routers controlled by attackers are known as bots, which commonly refer to software applications running as an automated task over the Internet network (Wikipedia, ``Botnet'')}}. 
% These Internet-connected devices are then used to mount a coordinated attack by relentlessly sending a large number of service requests to the target system. The overwhelming amount of traffic either slows the system to a stop or crashes it completely~\cite{mirkovic2004taxonomy,chang2002defending}. Such complicated and large-scale DDoS attacks, aimed at rendering targeted systems inoperative, are disruptive and pose a serious threat to network systems~\cite{KasperskyQ42019}.
% % [version 2]
% % Distributed Denial-of-Service (DDoS) attacks are well established as a significant threat to the network security of our present-day Internet, denying legitimate users access to shared and essential resources alike. 
% Distributed Denial-of-Service (DDoS) attacks are well established as a significant threat to our present-day Internet's network security, denying legitimate users access to shared and essential resources alike. The earliest reported DDoS attack in 1999~\cite{criscuolo2000distributed} started a wave of denial-of-service attacks that are distributed in nature. Even though more than a decade has since passed, these attacks---simple to set up, difficult to stop, and very effective---are more popular than ever as they stay potent yet straightforward~\cite{ISTR16-04}. The allocation of extra resources is a typical protective approach to handle such DDoS traffic. However, catering excess resources goes hand in hand with additional costs. There is a growing urgency to find a more practical and inexpensive alternative, clearly highlighted by the ongoing COVID-19 pandemic, which can effectively abate these disruptions by differentiating malicious traffic from the benign during an attack. It remains a hard problem to mitigate.
% % as it is crucial to differentiate malicious traffic from the benign during an attack instantaneously, it remains a hard problem to mitigate.
% % [version 3]
% Distributed Denial-of-Service (DDoS) attacks are well established as a significant threat to our present-day Internet's network security, denying legitimate users access to shared and essential resources alike. The earliest reported DDoS attack in 1999~\cite{criscuolo2000distributed} started a wave of denial-of-service attacks that are distributed in nature. Even though more than a decade has since passed, these attacks---simple to set up, difficult to stop, and very effective---are more popular than ever as they stay potent yet straightforward~\cite{ISTR16-04}. The allocation of extra resources is a typical protective approach to handle such DDoS traffic. However, catering excess resources goes hand in hand with additional costs. There is a growing urgency to find a more practical and inexpensive protective method, which can effectively abate these disruptions by differentiating malicious traffic from the benign during an attack. While it is not crucial for this method to achieve perfect accuracy, any reasonable differentiation process could potentially alleviate the huge strain on resources. We focus on devising such a defensive method.

% [version 4: Problem] Reduce and merge paragraph 2 to 1. Split into two paragraphs
Distributed Denial-of-Service (DDoS) attacks are well established as a significant threat to our present-day Internet network security, denying legitimate users access to shared and essential resources. The earliest reported DDoS attack in 1999~\cite{criscuolo2000distributed} started a wave of denial-of-service attacks that are distributed in nature. Even though more than two decades have passed, these attacks---simple to set up, difficult to stop, and very effective---are more popular than ever as they remain potent~\cite{ISTR16-04}.
% stay potent yet straightforward~\cite{ISTR16-04}. 
% One current popular method launches attacks by remotely controlling a network of well-organized and widely distributed Botnet devices in the application layer~\cite{8055579,SINGH2017344}, sending an overwhelming amount of traffic to the target system, and slowing the system to a stop. Such large-scale DDoS attacks are disruptive and pose a serious threat to network systems~\cite{KasperskyQ42019}.
% ======== [Motivation] ========
The allocation of extra resources is a typical protective approach to handle such DDoS traffic. However, catering excess resources goes hand in hand with additional costs. There is a growing urgency to find practical and inexpensive methods, which can effectively abate disruptions by filtering malicious traffic during an attack. 
% While it is not crucial for this method to achieve perfect accuracy, any reasonable differentiation process could potentially alleviate the huge strain on resources. We focus on devising such a filtering system.
While it is not crucial for this method to achieve perfect accuracy, any reasonable differentiation process could potentially alleviate the huge strain on resources. We focus on devising such a filtering system.




% % [2. Problem: application layer] \\
% One of the current methods popular with malicious agents is to launch an attack by remotely controlling a network of well-organized and widely distributed Botnet devices in the application layer. These devices are used to mount a coordinated attack by relentlessly sending a large number of service requests to the target system; sending an overwhelming amount of traffic that slows the system to a stop. Each bot in a botnet appears ``normal'' by making seemingly legitimate requests, making it difficult to distinguish between normal and attack traffic~\cite{8055579,SINGH2017344}. Such complicated and large-scale DDoS attacks, aimed at rendering targeted systems inoperative, are disruptive and pose a serious threat to network systems~\cite{KasperskyQ42019}.


% ======== [3. Motivation] ========
% % [version 1]
% DDoS detection, a primary form of defense mechanism, is facing growing difficulty in detecting malicious traffic as attacks are increasingly sophisticated in their approaches. In most cases, attackers disguise themselves as regular users by mimicking normal traffic. It is even possible that the underwhelming traffic in the early stages of an attack can be confused with as legitimate activities~\cite{peng2007survey}. Furthermore, attackers exploit fake (i.e., spoofed) IP addresses of enormous swarms of bots under their control, making it even harder for defense systems to recognize them~\cite{liu2009botnet}. The challenges of detecting DDoS attacks are as diverse as they are trying. 
% % [version 2]
% % Most existing anomaly detection mechanisms~\cite{peng2007survey,liu2009botnet}, a primary form of DDoS defense, are facing growing difficulty in detecting malicious traffic as application-layer attacks are increasingly sophisticated in their approaches. 
% A primary form of DDoS defense, anomaly detection mechanisms~\cite{peng2007survey,liu2009botnet}, is facing growing difficulty in detecting malicious traffic as application-layer attacks are increasingly sophisticated in their approaches. In many cases, evolving attackers alter their browsing behavior patterns to switch between request domains dynamically. It is even possible that the ever-changing attacker profiles and domain-switching tactics can be confused with legitimate activities. In this scenario, online machine learning seems to be an effective way to handle these evolving dynamics. Nevertheless, it is a challenging issue in the learning paradigm, as there are no accompanying ground truth labels of unidentified requests at the time of the attacks.
% % [version 3]
% A primary form of DDoS defense, anomaly detection mechanisms~\cite{peng2007survey,liu2009botnet}, faces growing difficulty in detecting malicious traffic as application-layer attacks are increasingly sophisticated in their approaches. There are several major challenges. First, the attacks are often domain-specific with different characteristics, making it hard for defense methods to generalize them. In many cases, evolving attackers alter their browsing behavior patterns to switch between request domains dynamically. It is even possible that the ever-changing attacker profiles and domain-switching tactics can be confused with legitimate activities. Second, while online machine learning seems to be an effective way to handle these evolving dynamics, the lack of ground truth labels of requests at the time of the attacks, required for supervised learning algorithms, poses another challenge for this learning paradigm. Third, the time constraint is a consideration in the online learning setting. Online models have to be computationally efficient to respond to requests rapidly during an on-going attack. We must address these challenges before deploying them in the real world.
% [version 4: Challenges]
A primary form of DDoS defense, anomaly detection mechanisms~\cite{peng2007survey,liu2009botnet}, faces growing difficulty in detecting malicious traffic as application-layer attacks are increasingly sophisticated. There are several significant challenges. First, the attacks are often domain-specific with varying characteristics, making it hard for defense methods to generalize them. Hence a two-class classifier trained on historic attacks might not be applicable to different victims. Second, the time constraint is a consideration in the real-time environment. Online models have to be computationally efficient to respond to requests rapidly during an on-going attack. Third, while online machine learning seems to be an effective way to handle these evolving dynamics, the lack of labeled requests at the time of the attacks, required for supervised learning algorithms, poses another challenge for this learning paradigm. We must address these challenges before deploying them in the real world.



% [4. Key examples] \\ 
% [version 1]
% % (1) DDoS Github in February 2018
% A recent example, in February 2018, GitHub experienced the largest DDoS attack ever recorded~\cite{kottler_2018}. The attack employed the amplification vector, which exploits a vulnerability in memcached instances to spoof IP addresses that targeted GitHub.com by sending much more data toward the target than the unspoofed source. The amplification attack using the memcached-based approach peaked at 1.35Tbps via 126.9 million packets per second.
% % (2) COVID-19 period DDoS
% Even more recently, there is a significant increase in both the quantity and quality of DDoS attacks that disrupted essential services during the COVID-2019 pandemic observed by Kaspersky in Q1 2020. There is an unexpected spike in the number of attacks;
% % (see \cref{fig:key}), 
% noticeable changes in the distribution of DDoS attacks by type, which doubled by $80\%$ against Q1 2019~\cite{KasperskyQ42019}. These examples illustrate the compelling need for quick and adaptive defense mechanisms as existing ones leave much to be desired.
% %The existing defenses against DDoS attacks to date are still lacking and leave much to be desired.
% % [version 2]
% Well-publicized attacks on large corporations, such as a recent example in February 2018 when GitHub experienced the largest DDoS attack ever recorded~\cite{kottler_2018}, often make the headlines. The attack using the Memcached-based approach peaked at 1.35Tbps via 126.9 million packets per second. While these attacks are astounding, Symantec’s telemetry shows that it is often small and medium-sized retailers, selling goods ranging from clothing to gardening equipment to medical supplies, that are on the receiving end of the majority of attacks~\cite{ISTR19-02}. It is a serious global issue that could potentially affect any business that operates online, especially the essential services during critical times, such as the COVID-2019 pandemic. Observed in Q1 2020, there is an unexpected spike in the number of attacks; noticeable changes in the distribution of DDoS attacks by type doubled by $80\%$ against Q1 2019~\cite{KasperskyQ42019}. It reveals the vital need for adaptive and effective DDoS defense systems.


% ======== [5. Existing work: Statistical and ML approach] ========
% % [version 1]
% In general, existing DDoS defenses take either one of two main approaches: (1) statistical anomaly-based detection or (2) machine learning-based detection. Statistical methods broadly involve some statistical measure of network traffic properties, such as entropy scoring of network packets~\cite{7345297,6601602,8256833,8466805}, IP filtering~\cite{1204223,Peng02detectingdistributed}, and IP source traceback~\cite{10.1007/3-540-36159-6_4,5467062}. These methods are limited in keeping up with new attacks and constrained by the need to define thresholds prior to the attacks. On the other hand, deep machine learning for DDoS detection can be broadly categorized into two main groups---those that are based on Recurrent Neural Network (RNN) architectures~\cite{8066291,10.1007/978-3-030-00018-9_15,doi:10.1002/dac.3497} and models that use Convolutional Neural Networks (CNNs)~\cite{Doriguzzi_Corin_2020,8416441}. The RNN-based methods have demonstrated superior detection capabilities on some sophisticated attacks for intrusion detection tasks, achieving a higher detection rate compared to other machine learning methods~\cite{8066291,10.1007/978-3-030-00018-9_15,doi:10.1002/dac.3497,Tann2018TowardsSS}.
% % [version 2]
% Existing DDoS defenses generally take either one of two main approaches---statistical anomaly-based detection or machine learning-based detection. Statistical methods broadly involve some statistical measure of network traffic properties, such as entropy scoring of network packets~\cite{7345297,6601602,8256833,8466805}, IP filtering~\cite{1204223,Peng02detectingdistributed}, and IP source traceback~\cite{10.1007/3-540-36159-6_4,5467062}. These methods are limited in keeping up with new attacks and constrained by the need to define thresholds prior to the attacks. On the other hand, we can broadly categorize deep machine learning for DDoS detection into two main groups: (1) methods~\cite{8066291,doi:10.1002/dac.3497,Yuan2017DeepDefenseID,8666588,Doriguzzi_Corin_2020,8416441,DANESHGADEHCAKMAKCI2020102756} that adopt an offline learning approach, where all attack data is observed and available for training the models, and (2) models~\cite{lima2019smart,7987186,DANESHGADEHCAKMAKCI2020102756} that only receive data, as more attack traffic is observed with time, performing incremental updates in an online manner. Many supervised DDoS detection methods, using label information in an offline environment, have been reported to achieve high detection accuracy in recent years. However, these models are slow to train, and require access to the entire attack data set and an a priori knowledge of the labels. It is not clear how to apply them to practical scenarios without labels during attacks.
% prediction. doi:10.1002/dac.3497 ; Yuan2017DeepDefenseID

% [version 3: Existing, online vs offline]
Existing DDoS defenses generally can be classified as statistical-based or machine learning-based detection. Statistical methods typically involve some fast calculation of network traffic properties, such as entropy scoring of network packets~\cite{7345297,6601602,8256833,8466805}, IP filtering~\cite{1204223,Peng02detectingdistributed}, and IP source traceback~\cite{10.1007/3-540-36159-6_4,5467062}. 
On the other hand, deep learning exploits intrinsic properties but could be computationally intensive. Most deep learning approaches for DDoS in the literature adopt offline learning, where the training is conducted much earlier (e.g., at least a few days) before the attack commences~\cite{8066291,doi:10.1002/dac.3497,Yuan2017DeepDefenseID,8666588,8416441}.
% Although many proposed offline learning methods reported high detection accuracy, these models are slow to train, require access to the entire attack dataset, and an a priori knowledge of the labels, and thus are not applicable in online scenarios.
There are fewer works on online learning that performs incremental updates as more attack requests arrive. {Çakmakçı} et al. gave an up-to-date survey of online DDoS detection~\cite{DANESHGADEHCAKMAKCI2020102756}. Most online learning methods employed unsupervised clustering (e.g., k-means) on the attack day data~\cite{lima2019smart,7987186,DANESHGADEHCAKMAKCI2020102756}. However, the optimization goal of these methods is not clear.


% Online learning faces computation constrains and the availability of labelled data.



% we can broadly categorize deep machine learning for DDoS detection into two main groups: (1) methods~\cite{8066291,doi:10.1002/dac.3497,Yuan2017DeepDefenseID,8666588,Doriguzzi_Corin_2020,8416441,DANESHGADEHCAKMAKCI2020102756} that adopt an offline learning approach, where all attack data is observed and available for training the models, and (2) models~\cite{lima2019smart,7987186,DANESHGADEHCAKMAKCI2020102756} that only receive data as more attack traffic is observed with time, performing incremental updates online. 

% ======== [add paragraph: optimization problem, online setting, notations] ========
% % [version 1]
% In an online setting, a dataset $\mathcal{D} = (\mathcal{N}, \mathcal{M})$ with two operational periods consists of (1) normal traffic data $\mathcal{N}$ and (2) attack data $\mathcal{M}  = \{M_1, M_2, \dots, M_T \}$, which is a mixture of legitimate and malicious traffic. An ideal method should first learn the characteristics of normal traffic from the normal dataset $\mathcal{N}$. Then, as an attack happens, this method has to rapidly learn from each batch $A_t$ of attack traffic at every timestep $t$ to improve its accuracy in identifying malicious traffic. 
% [version 2: formulate problem]

In this paper, we explore how deep learning can be leveraged to enhance performance, especially in the application-layer traffic, which exhibits intrinsic statistical properties. 
We first formulate a machine learning optimization problem, which utilizes data from two operational periods, normal-day traffic $\mathcal{N}$, and the attack-day traffic $\mathcal{M}$ that contains a mixture of unlabeled legitimate and malicious traffic. We assume that there is a rough estimate $\alpha$ of the proportion of attack requests in $\mathcal{M}$. The learning objective is a two-class classifier that can accurately predict requests from $\mathcal{N}$ as normal, and $\alpha$ proportion of requests in $\mathcal{M}$ as attacks.

    %---------------------------
    \begin{figure}[tbp]
        \centering
        \includegraphics[width=.5\linewidth]{image/PAN2}
        \caption{%The PAN framework 
        A framework that utilizes both ${\mathcal N}$ and ${\mathcal M}$ to rank network traffic based on their final $n_x / d_x$ scores. The higher the final score, the more likely the traffic is normal. To achieve computation speedup, the embedding of $N$ is transferred to $D$.
        }
        \label{fig:danframework}
    \end{figure}        
    %% %---------------------------

While the learning goal is well-defined, it is not clear how to attain it, especially with the constraints on computational resources. To solve the problem, our main idea is to extend one-class unsupervised learning in a two-step process. (1) We apply unsupervised learning on the normal-day traffic $\mathcal{N}$ to obtain a model $N$ that learns the distribution $P_n$ of $\mathcal{N}$. (2) When an attack commences, a similar unsupervised learning model $D$ rapidly learns the distribution $P_d$ of the mixture $\mathcal{M}$. Now, intuitively, the attack and normal requests can be differentiated based on the differences between two distributions $P_n$ and $P_d$. We employ techniques in PacketScore~\cite{1354679} that rank each request $x$ by $P_n(x)/P_d(x)$, where a higher score indicates a higher chance of an attack, as illustrated in Figure~\ref{fig:danframework}. In our construction, both models $N$ and $D$ are LSTM recurrent neural networks, designed for application-layer DDoS, where a ``request'' consists of a sequence of events (e.g., an \texttt{HTTP GET} to the landing page, followed by subsequent \texttt{HTTP GET} requests). To meet the online requirements, we design model $D$ to achieve quick online updates by relying on transfer learning. When an attack occurs, the optimized embedding of $N$ is transferred to $D$, significantly reducing the training needed for $D$. We call this particular construction of online learning the \textit{N-over-D} nets. %\textit{Associate Nets}.
% \textit{Predictive Associate Nets} (PAN).

Even though \textit{N-over-D} meet the online requirements, theoretically, it might not attain optimality in the proposed optimization problem. We design an online iterative two-class classifier for our proposed optimization problem. This online classifier does not have the ground truth label information. It uses pseudo-ground-truth labels, taking all traffic during attacks as malicious and labeling them accordingly. 
% We train the classifier using these inexact labels to improve iteratively with the $N$ and $D$ in \textit{associate nets} as a starting point. This enhanced iterative classification approach exploits all the normal and attack data, achieving remarkable detection performance. While it cannot be deployed in the online environment, it could still be useful in practice when the goal is to classify unlabeled historic $\mathcal{M}$. 
We train the classifier, with a similar model architecture as the $N$ and $D$ in \textit{N-over-D}, using these inexact labels to improve iteratively. This enhanced iterative classification approach achieves remarkable detection performance. While it is more suitable for attacks with an extended timeframe as it takes a longer training time, it could still be useful in practice when the goal is to classify unlabeled historic $\mathcal{M}$. 
 

    % %---------------------------
    % \begin{figure}[tbp]
    %     \centering
    %     \includegraphics[width=.85\linewidth]{image/ddosreportQ1_2020.png}
    %     \caption{Reported worldwide DDoS attacks in Q1 2020 during the COVID-2019 pandemic increased by $80\%$ from the previous year. The report observed a significant increase in both the quantity and quality of DDoS attacks. The attacks also demonstrated an apparent rise in both the average and maximum duration (figure from~\cite{KasperskyQ42019}). 
    %     % Reprinted from \textit{DDoS attacks in Q1 2020}, by Kaspersky Lab., May 6 2020~\cite{KasperskyQ42019}. 
    %     }
    %     \label{fig:key}
    % \end{figure} 
    % %% %---------------------------
    
% % [RNNs] \\
% \textit{Recurrent Neural Networks} (RNNs), a class of machine learning methods that models sequential information, have gained popularity over recent years leading to significant advances in Natural Language Processing (NLP)~\cite{Yao2013RecurrentNN,mesnil2013investigation,7472159} and Time Series Analysis~\cite{8141873,8467310,8126078}. A powerful variant of the RNN, the \textit{Long Short-Term Memory Neural Network} (LSTM)~\cite{10.1162/neco.1997.9.8.1735}, has achieved impressive performance in NLP tasks such as spoken language understanding~\cite{yao2014spoken,7953243}, machine translation~\cite{yao2015depthgated,wu2016googles}, and speech recognition~\cite{10.1145/3020078.3021745,Soltau_2017}. While the use of RNNs is starting to gain broader acceptance in the cybersecurity field, this machine learning method has pushed the state-of-the-art performances in many security applications. These applications include vulnerability detection~\cite{Tann2018TowardsSS,Li_2018,10.1145/3133956.3138840,grieco2016toward}, network traffic analysis~\cite{KIM201866,7785326,8466367}, and intrusion detection in industrial control systems~\cite{8023128}. The flexibility and generalizability of LSTMs in various security applications combined with its high performance motivate our work in using LSTMs for online DDoS defense. We propose a new DDoS defense framework that leverages these strengths.%sidesteps these difficulties. 


% [6. Our work, How it addresses challenges of the problem] \\
% % [version 1]
% Our proposed machine learning DDoS defense framework, the \textit{Defensive Authentication Networks} (DeAN), DDoS predictive model $D$ is partnered with an ally: a normal model $N$ that learns the data distribution of normal network traffic to determine the normality of a request (see \cref{fig:danframework}). The DDoS model can be thought of as analogous to a master art forger, trying to determine how closely an artwork resembles a replica, while the normal model is analogous to the original artist, trying to evaluate the authenticity of the artwork. Cooperation in this game drives both sides to improve their methods until the authenticity of artworks can be determined with high accuracy.
% % [version 2]
% Our proposed augmented anomaly detection DDoS defense framework, the \textit{Predictive Associate Networks} (PAN), partners an online learning DDoS predictive model $D$ with an ally: a normal model $N$ that learns the data distribution of normal network traffic to determine the normality of a request (see \cref{fig:danframework}). The DDoS model can be thought of as analogous to a master art forger, trying to determine how closely an artwork resembles a replica, while the normal model is analogous to the original artist, trying to evaluate the authenticity of the artwork. Cooperation in this game drives both sides to improve their methods until the authenticity of artworks can be determined with high accuracy.

% % [7. Contributions] \\
% This framework allows specific training algorithms for many types of DDoS defense models and algorithms. In this paper, we explore the particular case where the denominator $D$ evaluates DDoS traffic using an online LSTM model and a histogram, and the numerator $N$ is also an LSTM architecture aided by a histogram. We refer to this particular case as \textit{associate nets}. In this case, we can train $N$ and $D$ models using the highly successful backpropagation algorithm in machine learning algorithms and robust approximate frequency distribution statistical methods. We introduce and develop a DDoS detection framework designed for adaptive and effective attack mitigation, employing two collaborative LSTM recurrent neural networks and histograms to distinguish disruptive DDoS from legitimate regular traffic.


% ======== [combine paragraph 6 and 7. Online N/D solution.] ========
% % [version 1]
% Next, we propose an unsupervised online-learning anomaly detection framework, \textit{Predictive Associate Nets} (PAN), which partners an online predictive model $D$ that learns the attacks with an ally: model $N$ that learns the data distribution of normal network traffic, to determine the normality of a request (see \cref{fig:danframework}). This framework allows specific training algorithms for many types of DDoS defense models and algorithms. 
% In this paper, we explore the particular case where the denominator $D$ evaluates DDoS traffic using an online LSTM model and a histogram, and the numerator $N$ is also an LSTM architecture aided by a histogram. We refer to this particular case as \textit{associate nets}. 
% % In this case, we designed model $D$ to perform quick online updates by reducing it to a one-layer LSTM model, increasing the model efficiency. Furthermore, by transferring the optimized embedding of $N$ to $D$ during an attack, we significantly reduced the training needed for $D$.
% In this case, we design model $D$ to perform quick online updates. First, we can increase the model efficiency by reducing $D$ to a one-layer LSTM model. Second, we carry out transfer learning by imparting the optimized embedding of $N$ to $D$ when an attack occurs, significantly reducing the training needed for $D$. Employing two collaborative LSTM recurrent neural networks, we introduce an online detection framework designed for effective DDoS attack mitigation.
% % In this case, we can train $N$ and $D$ models using the highly successful backpropagation algorithm in machine learning algorithms and robust approximate frequency distribution statistical methods. 
% % We introduce and develop a DDoS detection framework designed for adaptive and effective attack mitigation, employing two collaborative LSTM recurrent neural networks and histograms to distinguish disruptive DDoS from legitimate regular traffic.
% [version 2: one direction]

%{\scriptsize Next, we propose an unsupervised online anomaly detection approach, \textit{Predictive Associate Nets} (PAN), which partners two predictive models to determine the legitimacy of requests. A model $N$ learns the data distribution of normal network traffic from $\mathcal{N}$, while an online model $D$ learns the distribution of the mixture traffic $\mathcal{M}  = \{M_1, M_2, \dots, M_T \}$ from each batch $M_t$ observed at every time interval $t$. This framework (see \cref{fig:danframework}), inspired by an online statistical detection method~\cite{1354679}, allows specific training algorithms for many types of DDoS defense models and algorithms. In this paper, we explore the particular case where both models $N$ and $D$ are LSTM recurrent neural networks. We refer to this particular case as \textit{associate nets}. In this case, we design model $D$ to achieve quick online updates by relying on transfer learning. When an attack occurs, the optimized embedding of $N$ is transferred to $D$, significantly reducing the training needed for $D$. Employing two collaborative predictive models, we introduce an online detection framework designed for effective DDoS attack mitigation.}

% ======== [add paragraph: classifier, enhanced, Baseline] ========
% % [version 1]
% To thoroughly evaluate our proposed online method, we first establish an upper bound by using an offline classifier that trains on the entire dataset $\mathcal{D}$ with actual ground truth labels to achieve the performance with full information. We also design another classification model that iteratively improves upon itself using pseudo labels, where all traffic during an attack is labeled as malicious. It does not have the ground truth label information. We then evaluate the performance of model $N$, trained only on normal traffic.  Finally, we establish the baseline model, offline $N/D$, inspired by an online statistical detection method~\cite{1354679}, which performs much better than the $N$ model. The methods described above take an offline approach and exploit all data, normal and attack, for training.
% [version 2: another direction]




% ======== [8. Experiments & Contributions] ========\\
% % [version 1]
% Our work demonstrates the ability of \textit{associate nets} to detect and mitigate a variety of DDoS attack schemes using a cooperative online learning approach that is flexible and robust. We find that it is advantageous to employ independent models that are united in discerning DDoS from regular traffic. We hope that our proposed framework will renew the interest in learning-based DDoS defense that are feasible in real-world deployment, and enable practical coordinated responses to the continually evolving DDoS attacks.
% [version 2]
Comprehensive experiments demonstrate the ability of our approach to mitigate a range of DDoS attacks. For example, in the \textit{CICIDS2017} dataset (LOIC attack), while the $N$ model achieves (32.57\%, 69.97\%) accuracy and false-positive rate, both the online \textit{N-over-D} and iterative classifier models accomplish marked improvements (93.3\%, 0.47\%) and (97.13\%, 0.65\%), respectively (see \cref{sec:experiments} for details). \\
% The results of our approach are very close to that of the full offline classifier (94.89\%, 0.37\%) that uses actual ground truth labels (see \cref{sec:experiments} for details). 
%We find that it is advantageous to employ independent models united in discerning DDoS from regular traffic. We hope that our proposed framework will renew the interest in learning-based DDoS defenses that are feasible in real-world deployment, and enable practical modern responses to the continually evolving DDoS attacks.

\noindent\textbf{Contribution.} 
\begin{enumerate}
\item We formulate DDoS detection on unlabeled data as a machine learning optimization problem with normal day ${\mathcal N}$, mixture ${\mathcal M}$, and the estimated $\alpha$ as training input. 

\item To meet the online requirement, we proposed an approach that extends from a one-class unsupervised learning method. We propose \textit{N-over-D}, which deploys an LSTM-based model on ${\mathcal N}$ and ${\mathcal M}$ separately, and incorporates transfer learning to speedup training in the online setting. 

\item We propose an iterative method to solve the proposed optimization problem in the online setting. 
\end{enumerate}


% [9. Organization] \\
% \textbf{Organization.} We organize the rest of the paper by first introducing the background information and challenges of the DDoS problem in Sec. \ref{sec:background}. In Sec. \ref{sec:dan}, we detail the framework with respect to the network traffic processing and our defense framework. We then describe the datasets used in our experiments in Sec. \ref{sec:datasets}. Next, we evaluate \textsc{auth nets} on these datasets and compare it with the state-of-the-art approaches in Sec. \ref{sec:experiments}. The performance analysis of our mitigation process is provided in Sec. \ref{sec:analysis}. Finally, we discuss several practical issues in Sec. \ref{sec:discuss}, summarize related work in Sec. \ref{sec:relatedwork}, and then conclude the paper in Sec. \ref{sec:conclude}.
\noindent\textbf{Organization.} We organize the rest of the paper by first introducing the background information and challenges of the DDoS problem in \cref{sec:background}. We formulate the problem in \cref{sec:formulate} and propose an appropriate approach in \cref{sec:pan}. We then detail the iterative classification method in \cref{sec:iterative} and the online framework of our approach in \cref{sec:associate}. 
In \cref{sec:experiments}, we describe the datasets used in our experiments and evaluate our approaches on these datasets, comparing them with state-of-the-art methods. We also analyze the performance of our mitigation process and discuss several practical issues. Finally, we summarize related work in \cref{sec:relatedwork} and conclude the paper in \cref{sec:conclude}.

